Loss it right: Euclidean and Riemannian Metrics in Learning-based Visual Odometry

This paper overviews different pose representations and metric functions in visual odometry (VO) networks. The performance of VO networks heavily relies on how their architecture encodes the information. The choice of pose representation and loss function significantly impacts network convergence and generalization. We investigate these factors in the VO network DeepVO by implementing loss functions based on Euler, quaternion, and chordal distance and analyzing their influence on performance. The results of this study provide insights into how loss functions affect the designing of efficient and accurate VO networks for camera motion estimation. The experiments illustrate that a distance that complies with the mathematical requirements of a metric, such as the chordal distance, provides better generalization and faster convergence. The code for the experiments can be found at https://github.com/remaro-network/Loss_VO_right

==> sections/aux.tex <==

\subsection{Riemannian manifolds}
A differentiable manifold is a smooth multidimensional curved surface that is locally Euclidean. This allows to locally approximate the manifold around a point $u$ through the tangent space $T_u\Omega$. The collection of all tangent spaces is the tangent bunle $T\Omega$. To measure lengths and angles between vectors in the tangent space, we need to give the tangent space additional structure, expressed as a positive-definite bilinear function []. Such a function is called a Riemannian metric, and can be thought of as an inner product of the tanget space, which is a expression of the angle between any two tangent vectors. The metric also induces a norm, allowing to locally measure lengths of vectors. A manifold equiped with a metric is a Riemannian manifold, and the properties that can be expressed entirely in terms of the metric are said to me intrinsic.
Riemannian manifolds can be embedded in the Euclidean space, by using the Euclidean space to induce a Riemannian metric. Two different isometric realisations of a Riemannian metric are possible.
\paragraph{Geodesics}
The geodesic is the curve of minimum length connecting the points $u$ and $v$.
On manifolds, we cannot directly add or substract two points $u,v \in \Omega$. Though they have same dimensions, they belong to different spaces, e.g. $X \in T_u\Omega$ and $Y \in T_v\Omega$, thus not directly comparable. Geodesics provide mechanisms to move vectors from one point to another, in the following way:  let $\gamma$ be a geodesic connecting points $u = \gamma(0)$ and $v = \gamma(T)$, and let $X \in T_u\Omega$. We can define a set of tangent vectors along the geodesic, $X(t) \in T_{\gamma(t)}\Omega$ such that the length of $X(t)$ and the angle (expressed through the Riemannian metric) between it and the velocity vector of the curve is constant. As a result, we get a unique vector $X(T) \in T_v\Omega$ at the endpoint $v$. \textbf{This mapping is called parallel transport or connection}.
When $\gamma_X(t)$ is defined for all $t>=0$, the manifold is said to be geodesically complete. 
The definition of a geodesic provided a point and a direction gives a natural mapping from (a subset of) the tangent space $T_u\Omega$ to $\Omega$ called the \textbf{exponential map} $\exp :B_r(0) \subset T_u\Omega \rightarrow \Omega$, which is defined by taking a unit step along the geodesic in the direction $X$, i.e. $\exp_u(X)=\gamma_X(1)$. The exponential map $exp_u$ is a local diffeomorphism, as it deforms the neighborhood $B_r(0)$ (a ball of radius $r$) of the origin on $T_u\Omega$ into a neighborhood of $u$.
The [] theorem guarantees hat geodesically complete manifolds are also complete metric spaces, in which one can realise a distance (called geodesic distance or metric) between any pair of points $u,v$ as the length of the shortest part between them.
Isometries are distance-preserving maps between metric spaces, i.e. they preserve geodesic distances.


\paragraph{Metric over a Lie algebra u(n)}
Let $\mathfrak{u}(n)$ be the Lie algebra of the Lie group U(n). I can define a positive-definite inner product over $\mathfrak{u}(n)$ in this way: if $A,B \in \mathfrak{u}(n)$ I define 
\begin{equation}
    \langle A,B \rangle := \Re(\operatorname{Tr}(AB^*)),
\end{equation}
where by $\Re$ I denote the real part and by $B^*$ the conjugate transpose of $B$. Why does this inner product over $\mathfrak{u}(n)$ define the unique left-invariant metric on the Lie group U(n)?%https://math.stackexchange.com/questions/448803/metric-over-a-lie-algebra-mathfrakun
%https://math.stackexchange.com/questions/2062811/constructing-a-metric-on-a-lie-group

Let $A$ and $B$ be complex $n\times n$ matrices with respective $(j,k)$ entries $A_{jk}$ and $B_{jk}$, and note that $B^*$ is the conjugate transpose, i.e has $(j,k)$ entry $\bar{B}_{kj}$. Bu definition,
\begin{equation}
    \langle A, B\rangle
  = \Re\bigl(\text{Tr}(AB^*)\bigr)
  = \Re \sum_{j,k=1}^n A_{jk} \bar{B}_{jk},
\end{equation}
which is the Euclidean inner product of $A$ and $B$ if these matrices are identified with complex vectors in $C^{n^2}$.

\section{Unconstraining the optimization}
One classic method is \textit{parameterization}. Parameterization is the process of transforming your constrained optimization problem into an unconstrained optimization problem by representing your variables in a different way. For Euler angles, this has been done bu parameterizing them as quaternions.
The other method is via Lie algebra representation. Once we have our Euler angles represented as a vector in se(3), we can use this representation in our optimization problem. Instead of optimizing over the Euler angles themselves, we can optimize over the corresponding vector in the se(3) space. This gives us an unconstrained optimization problem that we can solve using standard optimization techniques.

In order to measure the distance between two vectors represented in the Lie algebra se(3), we can use the concept of the exponential map.

The exponential map is a function that maps elements of the Lie algebra to elements of the group. In the case of SE(3), the exponential map takes a vector of six parameters (three for translation and three for rotation) in the Lie algebra se(3) and maps it to a homogeneous transformation matrix in SE(3) that represents a rigid body motion.

To measure the distance between two vectors in se(3), we can first use the exponential map to convert them into corresponding transformation matrices in SE(3). We can then measure the distance between these transformation matrices using any appropriate metric, such as the Frobenius norm or the geodesic distance on the manifold.
